GLAD: Global-Local View Alignment and Background Debiasing for Unsupervised Video Domain Adaptation with Large Domain Gap

In this work, we tackle the challenging problem of unsupervised video domain adaptation (UVDA) for action recognition. We specifically focus on scenarios with a substantial domain gap, in contrast to existing works primarily deal with small domain gaps between labeled source domains and unlabeled target domains. To establish a more realistic setting, we introduce a novel UVDA scenario, denoted as Kinetics->BABEL, with a more considerable domain gap in terms of both temporal dynamics and background shifts. To tackle the temporal shift, i.e., action duration difference between the source and target domains, we propose a global-local view alignment approach. To mitigate the background shift, we propose to learn temporal order sensitive representations by temporal order learning and background invariant representations by background augmentation. We empirically validate that the proposed method shows significant improvement over the existing methods on the Kinetics->BABEL dataset with a large domain gap. The code is available at https://github.com/KHUVLL/GLAD.

==> table/ek_main.tex <==
\begin{table}[t]
\centering
% \caption{\textbf{Results on the Epic-Kitchens.}}
\caption{\textbf{Comparison with the state-of-the-art on the Epic-Kitchens dataset.} We show the mean class accuracy (MCA).  we indicate the input modalities used by each model: ``R'' indicates RGB, and ``F'' indicates the flow modality. All methods employ I3D~\cite{carreira2018i3d} as the backbone. The best performance is in \best{bold} and the second best is \second{underscored}.}

\label{tab:main_k-babel}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|cccccc|c}
      \toprule
      \multirow{2}{*}{Method} &\multirow{2}{*}{Modality}& \multicolumn{7}{c}{Epic-Kitchens} \\
    \cmidrule(lr){3-9}
      && D2$\rightarrow$D1 & D3$\rightarrow$D1 & D1$\rightarrow$D2 & D3$\rightarrow$D2 & D1$\rightarrow$D3 & D2$\rightarrow$D3 & Avg \\
      \midrule
      Source Only& R & 35.4 & 34.6& 32.8& 35.8 &34.1& 39.1& 35.3 \\
      Source Only (mm)&R+F &  42.5& 44.3 &42.0& 56.3& 41.2& 46.5& 45.5 \\
      
      \midrule
      
      DANN~\cite{dann}&\multirow{5}{*}{R} &38.3 & 38.8& 37.7 &42.1 &36.6& 41.9 &39.2 \\
      TA3N~\cite{chen2019ta3n} &&40.9& 39.9& 34.2& 44.2& 37.4& 42.8& 39.9 \\
      CoMix~\cite{sahoo2021comix} &&38.6& 42.3& 42.9 &49.2& 40.9& 45.2&43.2 \\
      TranSVAE~\cite{wei2022transvae} &&50.3 & 48.0& 50.5 & 58.0 & 50.3& 58.6 &52.6 \\
      Ours && 37.5 $\pm$ 1.2 & 36.7 $\pm$ 1.1 & 40.8 $\pm$ 0.9 & 42.0 $\pm$ 0.7 & 37.8 $\pm$ 0.7 & 39.6 $\pm$ 0.2 \\
      
      \midrule
      CMCo~\cite{kim2021CMCo}&\multirow{4}{*}{R+F}  &49.5& 51.5& 50.3 &56.3 &46.3 &52.0 &51.0\\
      STCDA~\cite{song2021STCDA} &&49.0 &52.6 &52.0 &55.6& 45.5 &52.5& 51.2\\
      MM-SADA~\cite{munro2020mm-sada} &&48.2 &50.9& 49.5& 56.1 &44.1 &52.7 &50.3 \\
      
      CIA~\cite{yang2022cia} &&52.5&  47.8&  49.8&  53.2 & 52.2&  57.6 & 52.2 \\
      \midrule
      Supervised Target &R& 57.0 & 57.0 & 64.0 & 64.0 & 63.7 & 63.7 & 61.5  \\
      Supervised Target (mm) &R+F& 62.8 &62.8& 71.7& 71.7& 74.0& 74.0& 69.5  \\
      \bottomrule
  \end{tabular}%
}

\label{tab:main_ek}
\end{table}



==> table/ucf-hmdb_main.tex <==
\begin{table}[htbp]
\centering
\label{tab:main_ucf-hmdb}
% \centering 
% \caption{\textbf{Results on UCF-HMDB.} We show the Top-1 accuracy for the UCF-HMDB dataset. }
\caption{\textbf{Comparison with the state-of-the-art on the UCF-HMDB dataset.} We show the overall Top-1 accuracy for the UCF-HMDB dataset. The best performance is in \best{bold} and the second best is \second{underscored}.}

\resizebox{\linewidth}{!}{%
\begin{tabular}{ l |c | c | c | c }
      \toprule

Method & Backbone& UCF$\rightarrow$HMDB & HMDB$\rightarrow$UCF & Average \\
      \midrule

% Sup-SourceOnly & ResNet-101 & 71.7 & 73.9 & 72.8 \\
Source Only & I3D  & $80.3$ & $88.8$ & $84.5$ \\
Source Only (improved pretrained) & I3D  & 85.6 & 95.1 & 90.4 \\
Source Only (improved pretrained) & TSM  & 83.3 & 96.2 & 89.8 \\
      \midrule
DANN~\cite{dann} &\multirow{11}{*}{I3D} & $80.7$ & $88.0$ & $84.3$ \\
SAVA~\cite{choi2020sava} &&  $82.2$ & $91.2$ & $86.7$ \\
CoMix~\cite{sahoo2021comix}  & & 86.7& 93.9 & 90.3 \\
CO\textsuperscript{$2$}A~\cite{da2022co2a}  & & 87.8 & 95.8 & 91.8 \\
CIA(multi)~\cite{yang2022cia} &  & 92.0& 94.6 & 93.3 \\
TranSVAE~\cite{wei2022transvae}&   & 87.8& 99.0 & 93.4 \\
MM-SADA(multi)~\cite{munro2020mm-sada} &  & 84.2 & 91.1 &   87.7 \\
CMCo(multi)~\cite{kim2021CMCo} &  & 84.7 & 92.8 &   88.8 \\
STCDA~\cite{song2021STCDA}&   & 81.9 & 91.9 &    86.9 \\
ACAN~\cite{Xu_2022ACAN} &  & 85.4 & 93.8 &   89.6 \\

\textbf{Ours}& & 81.6 $\pm$ 0.9 &  93.4 $\pm$ 1.4 & 87.5  \\  % 18261 (ariel) / 18666 (ariel)
\textbf{Ours (best)}& & 83.1 & 96.0 & 89.6 \\  % 18703 (ariel) / 18144 (ariel)
      \midrule

TA\textsuperscript{$3$}N~\cite{chen2019ta3n}  & \multirow{3}{*}{TRN} & $81.4$ & $90.5$ & $85.9$ \\

ATCoN(source-free)~\cite{xu2022ATCoN}&   & 79.7 & 85.3 &   82.5 \\
TCoN~\cite{pan2019tcon} &  & 87.2 & 89.0 &  88.2 \\

      \midrule

MA\textsuperscript{$2$}L-TD~\cite{chen2022mal-td} & ResNet-101 & 85.0 & 86.6 &   85.8 \\
      \midrule

DVM~\cite{dvm} & \multirow{2}{*}{TSM} &  87.0 & 98.6 & 92.8 \\
\textbf{Ours}& & 86.4 & 95.5 &  \\

      \midrule
% Supervised Target& I3D & $95.0$ & $96.8$ & $95.9$ \\
Supervised Target& I3D & 95.6 & 99.8 & 97.7 \\
Supervised Target& TSM & 96.4 & 99.6 & 98.0 \\
      \bottomrule
\end{tabular}%
}

\end{table}

